SERENGETI: Massively Multilingual Language Models for Africa

Multilingual pretrained language models (mPLMs) acquire valuable, generalizable linguistic information during pretraining and have advanced the state of the art on task-specific finetuning. To date, only ~31 out of ~2,000 African languages are covered in existing language models. We ameliorate this limitation by developing SERENGETI, a massively multilingual language model that covers 517 African languages and language varieties. We evaluate our novel models on eight natural language understanding tasks across 20 datasets, comparing to 4 mPLMs that cover 4-23 African languages. SERENGETI outperforms other models on 11 datasets across the eights tasks, achieving 82.27 average F_1. We also perform analyses of errors from our models, which allows us to investigate the influence of language genealogy and linguistic similarity when the models are applied under zero-shot settings. We will publicly release our models for research.\footnote{\href{https://github.com/UBC-NLP/serengeti}{https://github.com/UBC-NLP/serengeti}}

==> Tables/jacc_sim.tex <==
\begin{table*}[]
\small
\resizebox{0.63\textwidth}{!}{%
\begin{adjustbox}{angle=90}
\begin{tabular}{llllllllllllllllllllllllllllllllllll}
    & afr  & amh  & bam  & bbj  & ewe  & fon  & gax  & gaz  & hau  & ibo  & kin  & lug  & luo  & mlg  & mos  & nbl  & nso  & nya  & orm  & pcm  & run  & sna  & som  & sot  & ssw  & swh & tir  & tsn  & tso  & twi  & ven  & wol  & xho  & yor  & zul  \\
afr & 1    & 0.27 & 0.03 & 0.09 & 0.20 & 0.13 & 0.16 & 0.09 & 0.41 & 0.37 & 0.34 & 0.38 & 0.22 & 0.41 & 0.15 & 0.28 & 0.35 & 0.26 & 0.34 & 0.13 & 0.25 & 0.25 & 0.43 & 0.26 & 0.27 &     & 0.12 & 0.36 & 0.29 & 0.20 & 0.22 & 0.38 & 0.42 & 0.31 & 0.38 \\
amh & 0.27 & 1    & 0.03 & 0.09 & 0.19 & 0.14 & 0.15 & 0.10 & 0.25 & 0.30 & 0.25 & 0.27 & 0.19 & 0.30 & 0.15 & 0.22 & 0.27 & 0.21 & 0.27 & 0.15 & 0.21 & 0.20 & 0.31 & 0.23 & 0.22 &     & 0.28 & 0.24 & 0.24 & 0.20 & 0.19 & 0.26 & 0.27 & 0.25 & 0.28 \\
bam & 0.03 & 0.03 & 1    & 0.13 & 0.09 & 0.12 & 0.09 & 0.11 & 0.02 & 0.05 & 0.04 & 0.03 & 0.08 & 0.04 & 0.11 & 0.06 & 0.06 & 0.07 & 0.03 & 0.12 & 0.06 & 0.07 & 0.04 & 0.08 & 0.07 &     & 0.08 & 0.03 & 0.07 & 0.09 & 0.08 & 0.03 & 0.03 & 0.05 & 0.05 \\
bbj & 0.09 & 0.09 & 0.13 & 1    & 0.24 & 0.32 & 0.16 & 0.14 & 0.08 & 0.14 & 0.12 & 0.1  & 0.2  & 0.14 & 0.29 & 0.16 & 0.17 & 0.17 & 0.09 & 0.28 & 0.17 & 0.17 & 0.12 & 0.21 & 0.17 &     & 0.13 & 0.09 & 0.18 & 0.23 & 0.21 & 0.11 & 0.1  & 0.15 & 0.13 \\
ewe & 0.20 & 0.19 & 0.09 & 0.24 & 1    & 0.36 & 0.29 & 0.20 & 0.19 & 0.31 & 0.26 & 0.23 & 0.38 & 0.29 & 0.34 & 0.32 & 0.36 & 0.37 & 0.20 & 0.37 & 0.34 & 0.34 & 0.27 & 0.43 & 0.35 &     & 0.23 & 0.19 & 0.40 & 0.51 & 0.38 & 0.23 & 0.24 & 0.31 & 0.30 \\
fon & 0.13 & 0.14 & 0.12 & 0.32 & 0.36 & 1    & 0.23 & 0.18 & 0.13 & 0.21 & 0.18 & 0.15 & 0.29 & 0.20 & 0.35 & 0.23 & 0.24 & 0.26 & 0.14 & 0.34 & 0.26 & 0.23 & 0.18 & 0.30 & 0.26 &     & 0.21 & 0.13 & 0.27 & 0.33 & 0.30 & 0.16 & 0.16 & 0.24 & 0.20 \\
gax & 0.16 & 0.15 & 0.09 & 0.16 & 0.29 & 0.23 & 1    & 0.44 & 0.15 & 0.22 & 0.20 & 0.19 & 0.30 & 0.22 & 0.28 & 0.26 & 0.26 & 0.28 & 0.20 & 0.27 & 0.27 & 0.27 & 0.25 & 0.30 & 0.26 &     & 0.16 & 0.14 & 0.28 & 0.30 & 0.30 & 0.18 & 0.18 & 0.23 & 0.23 \\
gaz & 0.09 & 0.10 & 0.11 & 0.14 & 0.20 & 0.18 & 0.44 & 1    & 0.08 & 0.13 & 0.11 & 0.11 & 0.20 & 0.13 & 0.23 & 0.16 & 0.15 & 0.17 & 0.12 & 0.23 & 0.17 & 0.17 & 0.15 & 0.20 & 0.16 &     & 0.13 & 0.08 & 0.17 & 0.21 & 0.19 & 0.11 & 0.1  & 0.14 & 0.13 \\
hau & 0.41 & 0.25 & 0.02 & 0.08 & 0.19 & 0.13 & 0.15 & 0.08 & 1    & 0.37 & 0.34 & 0.40 & 0.20 & 0.38 & 0.14 & 0.26 & 0.32 & 0.25 & 0.35 & 0.11 & 0.25 & 0.24 & 0.43 & 0.22 & 0.25 &     & 0.11 & 0.37 & 0.27 & 0.19 & 0.20 & 0.41 & 0.43 & 0.33 & 0.36 \\
ibo & 0.37 & 0.30 & 0.05 & 0.14 & 0.31 & 0.21 & 0.22 & 0.13 & 0.37 & 1    & 0.39 & 0.40 & 0.32 & 0.45 & 0.22 & 0.35 & 0.43 & 0.35 & 0.34 & 0.22 & 0.34 & 0.34 & 0.45 & 0.36 & 0.35 &     & 0.18 & 0.35 & 0.38 & 0.31 & 0.31 & 0.37 & 0.43 & 0.45 & 0.44 \\
kin & 0.34 & 0.25 & 0.04 & 0.12 & 0.26 & 0.18 & 0.20 & 0.11 & 0.34 & 0.39 & 1    & 0.41 & 0.30 & 0.40 & 0.19 & 0.37 & 0.40 & 0.37 & 0.30 & 0.19 & 0.46 & 0.36 & 0.42 & 0.33 & 0.36 &     & 0.16 & 0.31 & 0.38 & 0.27 & 0.29 & 0.32 & 0.41 & 0.34 & 0.44 \\
lug & 0.38 & 0.27 & 0.03 & 0.10 & 0.23 & 0.15 & 0.19 & 0.11 & 0.40 & 0.40 & 0.41 & 1    & 0.27 & 0.39 & 0.17 & 0.35 & 0.38 & 0.34 & 0.35 & 0.15 & 0.36 & 0.31 & 0.44 & 0.29 & 0.33 &     & 0.14 & 0.36 & 0.34 & 0.24 & 0.26 & 0.38 & 0.47 & 0.35 & 0.44 \\
luo & 0.22 & 0.19 & 0.08 & 0.20 & 0.38 & 0.29 & 0.30 & 0.20 & 0.20 & 0.32 & 0.30 & 0.27 & 1    & 0.31 & 0.31 & 0.39 & 0.38 & 0.42 & 0.22 & 0.36 & 0.40 & 0.39 & 0.30 & 0.43 & 0.39 &     & 0.22 & 0.21 & 0.41 & 0.40 & 0.42 & 0.23 & 0.27 & 0.31 & 0.34 \\
mlg & 0.41 & 0.30 & 0.04 & 0.14 & 0.29 & 0.20 & 0.22 & 0.13 & 0.38 & 0.45 & 0.40 & 0.39 & 0.31 & 1    & 0.22 & 0.35 & 0.44 & 0.35 & 0.35 & 0.21 & 0.34 & 0.34 & 0.47 & 0.37 & 0.35 &     & 0.18 & 0.36 & 0.39 & 0.30 & 0.31 & 0.38 & 0.42 & 0.40 & 0.44 \\
mos & 0.15 & 0.15 & 0.11 & 0.29 & 0.34 & 0.35 & 0.28 & 0.23 & 0.14 & 0.22 & 0.19 & 0.17 & 0.31 & 0.22 & 1    & 0.25 & 0.26 & 0.27 & 0.15 & 0.35 & 0.27 & 0.25 & 0.21 & 0.31 & 0.27 &     & 0.21 & 0.14 & 0.28 & 0.34 & 0.29 & 0.17 & 0.17 & 0.23 & 0.22 \\
nbl & 0.28 & 0.22 & 0.06 & 0.16 & 0.32 & 0.23 & 0.26 & 0.16 & 0.26 & 0.35 & 0.37 & 0.35 & 0.39 & 0.35 & 0.25 & 1    & 0.47 & 0.48 & 0.25 & 0.27 & 0.43 & 0.46 & 0.35 & 0.41 & 0.62 &     & 0.21 & 0.26 & 0.48 & 0.33 & 0.42 & 0.27 & 0.41 & 0.33 & 0.55 \\
nso & 0.35 & 0.27 & 0.06 & 0.17 & 0.36 & 0.24 & 0.26 & 0.15 & 0.32 & 0.43 & 0.40 & 0.38 & 0.38 & 0.44 & 0.26 & 0.47 & 1    & 0.42 & 0.31 & 0.27 & 0.39 & 0.39 & 0.42 & 0.55 & 0.47 &     & 0.21 & 0.38 & 0.51 & 0.37 & 0.40 & 0.33 & 0.42 & 0.40 & 0.50 \\
nya & 0.26 & 0.21 & 0.07 & 0.17 & 0.37 & 0.26 & 0.28 & 0.17 & 0.25 & 0.35 & 0.37 & 0.34 & 0.42 & 0.35 & 0.27 & 0.48 & 0.42 & 1    & 0.25 & 0.27 & 0.46 & 0.46 & 0.34 & 0.45 & 0.48 &     & 0.19 & 0.25 & 0.51 & 0.38 & 0.44 & 0.26 & 0.35 & 0.34 & 0.44 \\
orm & 0.34 & 0.27 & 0.03 & 0.09 & 0.20 & 0.14 & 0.20 & 0.12 & 0.35 & 0.34 & 0.30 & 0.35 & 0.22 & 0.35 & 0.15 & 0.25 & 0.31 & 0.25 & 1    & 0.14 & 0.25 & 0.24 & 0.42 & 0.24 & 0.25 &     & 0.15 & 0.30 & 0.27 & 0.21 & 0.21 & 0.35 & 0.35 & 0.30 & 0.33 \\
pcm & 0.13 & 0.15 & 0.12 & 0.28 & 0.37 & 0.34 & 0.27 & 0.23 & 0.11 & 0.22 & 0.19 & 0.15 & 0.36 & 0.21 & 0.35 & 0.27 & 0.27 & 0.27 & 0.14 & 1    & 0.26 & 0.28 & 0.19 & 0.35 & 0.30 &     & 0.32 & 0.13 & 0.29 & 0.37 & 0.35 & 0.14 & 0.15 & 0.23 & 0.21 \\
run & 0.25 & 0.21 & 0.06 & 0.17 & 0.34 & 0.26 & 0.27 & 0.17 & 0.25 & 0.34 & 0.46 & 0.36 & 0.40 & 0.34 & 0.27 & 0.43 & 0.39 & 0.46 & 0.25 & 0.26 & 1    & 0.44 & 0.35 & 0.40 & 0.43 &     & 0.19 & 0.24 & 0.44 & 0.36 & 0.38 & 0.26 & 0.33 & 0.32 & 0.40 \\
sna & 0.25 & 0.20 & 0.07 & 0.17 & 0.34 & 0.23 & 0.27 & 0.17 & 0.24 & 0.34 & 0.36 & 0.31 & 0.39 & 0.34 & 0.25 & 0.46 & 0.39 & 0.46 & 0.24 & 0.28 & 0.44 & 1    & 0.33 & 0.39 & 0.43 &     & 0.21 & 0.23 & 0.44 & 0.35 & 0.41 & 0.25 & 0.32 & 0.32 & 0.39 \\
som & 0.43 & 0.31 & 0.04 & 0.12 & 0.27 & 0.18 & 0.25 & 0.15 & 0.43 & 0.45 & 0.42 & 0.44 & 0.3  & 0.47 & 0.21 & 0.35 & 0.42 & 0.34 & 0.42 & 0.19 & 0.35 & 0.33 & 1    & 0.34 & 0.34 &     & 0.17 & 0.37 & 0.37 & 0.28 & 0.29 & 0.41 & 0.45 & 0.40 & 0.45 \\
sot & 0.26 & 0.23 & 0.08 & 0.21 & 0.43 & 0.30 & 0.3  & 0.20 & 0.22 & 0.36 & 0.33 & 0.29 & 0.43 & 0.37 & 0.31 & 0.41 & 0.55 & 0.45 & 0.24 & 0.35 & 0.40 & 0.39 & 0.34 & 1    & 0.43 &     & 0.24 & 0.27 & 0.52 & 0.44 & 0.46 & 0.26 & 0.31 & 0.35 & 0.41 \\
ssw & 0.27 & 0.22 & 0.07 & 0.17 & 0.35 & 0.26 & 0.26 & 0.16 & 0.25 & 0.35 & 0.36 & 0.33 & 0.39 & 0.35 & 0.27 & 0.62 & 0.47 & 0.48 & 0.25 & 0.30 & 0.43 & 0.43 & 0.34 & 0.43 & 1    &     & 0.22 & 0.25 & 0.50 & 0.35 & 0.44 & 0.26 & 0.38 & 0.33 & 0.52 \\
swh &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      &      & 1   &      &      &      &      &      &      &      &      &      \\
tir & 0.12 & 0.28 & 0.08 & 0.18 & 0.23 & 0.21 & 0.16 & 0.13 & 0.11 & 0.18 & 0.16 & 0.14 & 0.22 & 0.18 & 0.21 & 0.21 & 0.21 & 0.19 & 0.15 & 0.32 & 0.19 & 0.21 & 0.17 & 0.24 & 0.22 &     & 1    & 0.11 & 0.21 & 0.24 & 0.23 & 0.13 & 0.13 & 0.18 & 0.18 \\
tsn & 0.36 & 0.24 & 0.03 & 0.09 & 0.19 & 0.13 & 0.14 & 0.08 & 0.37 & 0.35 & 0.31 & 0.36 & 0.21 & 0.36 & 0.14 & 0.26 & 0.38 & 0.25 & 0.30 & 0.13 & 0.24 & 0.23 & 0.37 & 0.27 & 0.25 &     & 0.11 & 1    & 0.28 & 0.20 & 0.21 & 0.34 & 0.39 & 0.30 & 0.36 \\
tso & 0.29 & 0.24 & 0.07 & 0.18 & 0.40 & 0.27 & 0.28 & 0.17 & 0.27 & 0.38 & 0.38 & 0.34 & 0.41 & 0.39 & 0.28 & 0.48 & 0.48 & 0.51 & 0.27 & 0.29 & 0.44 & 0.44 & 0.37 & 0.52 & 0.50 &     & 0.21 & 0.28 & 1    & 0.40 & 0.47 & 0.29 & 0.37 & 0.36 & 0.48 \\
twi & 0.20 & 0.20 & 0.09 & 0.23 & 0.51 & 0.33 & 0.30 & 0.21 & 0.19 & 0.31 & 0.27 & 0.24 & 0.40 & 0.30 & 0.34 & 0.33 & 0.37 & 0.38 & 0.21 & 0.37 & 0.36 & 0.35 & 0.28 & 0.44 & 0.35 &     & 0.24 & 0.20 & 0.40 & 1    & 0.39 & 0.23 & 0.24 & 0.36 & 0.31 \\
ven & 0.22 & 0.19 & 0.08 & 0.21 & 0.38 & 0.30 & 0.3  & 0.19 & 0.20 & 0.31 & 0.29 & 0.26 & 0.42 & 0.31 & 0.29 & 0.42 & 0.40 & 0.44 & 0.21 & 0.35 & 0.38 & 0.41 & 0.29 & 0.46 & 0.44 &     & 0.23 & 0.21 & 0.47 & 0.39 & 1    & 0.22 & 0.27 & 0.30 & 0.35 \\
wol & 0.38 & 0.26 & 0.03 & 0.11 & 0.23 & 0.16 & 0.18 & 0.11 & 0.41 & 0.37 & 0.32 & 0.38 & 0.23 & 0.38 & 0.17 & 0.27 & 0.33 & 0.26 & 0.35 & 0.14 & 0.26 & 0.25 & 0.41 & 0.26 & 0.26 &     & 0.13 & 0.34 & 0.29 & 0.23 & 0.22 & 1    & 0.4  & 0.33 & 0.36 \\
xho & 0.42 & 0.27 & 0.03 & 0.10 & 0.24 & 0.16 & 0.18 & 0.10 & 0.43 & 0.43 & 0.41 & 0.47 & 0.27 & 0.42 & 0.17 & 0.41 & 0.42 & 0.35 & 0.35 & 0.15 & 0.33 & 0.32 & 0.45 & 0.31 & 0.38 &     & 0.13 & 0.39 & 0.37 & 0.24 & 0.27 & 0.40 & 1    & 0.36 & 0.56 \\
yor & 0.31 & 0.25 & 0.05 & 0.15 & 0.31 & 0.24 & 0.23 & 0.14 & 0.33 & 0.45 & 0.34 & 0.35 & 0.31 & 0.40 & 0.23 & 0.33 & 0.40 & 0.34 & 0.30 & 0.23 & 0.32 & 0.32 & 0.40 & 0.35 & 0.33 &     & 0.18 & 0.30 & 0.36 & 0.36 & 0.30 & 0.33 & 0.36 & 1    & 0.38 \\
zul & 0.38 & 0.28 & 0.05 & 0.13 & 0.30 & 0.20 & 0.23 & 0.13 & 0.36 & 0.44 & 0.44 & 0.44 & 0.34 & 0.44 & 0.22 & 0.55 & 0.50 & 0.44 & 0.33 & 0.21 & 0.40 & 0.39 & 0.45 & 0.41 & 0.52 &     & 0.18 & 0.36 & 0.48 & 0.31 & 0.35 & 0.36 & 0.56 & 0.38 & 1   
\end{tabular}
\end{adjustbox}}
\caption{Jaccard similarity measure between all languages in our benchmark. Jaccard similarity is a measure between $0$ and $1$.}
\label{tab:jacc_sim}
\end{table*}

==> Tables/other_information/NER.tex <==
\begin{table}[h!]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{3cm}p{2cm} p{1cm}}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Sent}} % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
\\
 \toprule
\multirow{}{} {\textbf{Masakhane-NER}}  & \textbf{Hausa} & $2,720$ \\ %& $0.453$\% & $0.448$\%\\
                                  & \textbf{Igbo} & $3,190$ \\
                                  & \textbf{Yoruba} & $3,035$ \\
                                  & \textbf{Amharic} & $2,500$\\
                                  & \textbf{Kinyarwanda} & $3,015$ \\
                                  & \textbf{Luo} & $921$\\
                                  & \textbf{Luganda} & $2,604$ \\
                                  & \textbf{Naija Pidgin} & $3,000$\\
                                  & \textbf{Swahili} & $3,006$ \\
                                  & \textbf{Wolof} & $2,674$ \\
                        %& $0.44$\%  &$0.419$\%  \\
                        \hline
\multirow{}{} {\textbf{WikiAnn}}   & \textbf{Yoruba}  &$31,086$\\%& $0.616$\% & $0.605$\% \\
                                  & \textbf{Akan}  &$31,086$\\
                                  & \textbf{Twi}  &$31,086$  \\
                                  & \textbf{Swahili}  &$31,086$   \\
                                  & \textbf{Amharic}  &$31,086$ \\
                                  & \textbf{Kinyarwanda}  &$31,086$ \\
                                  \hline
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{NCHLT}}   & \textbf{Zulu}  &$201,331$  \\%& $0.616$\% & $0.605$\% \\
                                  & \textbf{Xhosa}  &$121,166$  \\
                                  & \textbf{Sesotho}  &$269,624$ \\
                                  & \textbf{Siswati}  &$175,378$  \\
                                  & \textbf{Xitsonga}  &$268,496$ \\
                                  & \textbf{Sepedi}  &$201,431$  \\
                                  & \textbf{Ndebele}  &$161,544$  \\
                                  & \textbf{Afrikaans}  &$229,818$   \\
                                   & \textbf{Setswana}  &$231,390$  \\
                                    & \textbf{Tshivenda}  &$235,450$  \\
                                  \hline
\multirow{}{} {\textbf{DS NER}} & \textbf{Hausa} & $1,450$  \\ \\
\hline
\multirow{}{} {\textbf{Yoruba-Twi NER}} & \textbf{Yoruba} & $1,168$  \\ \\ \\
 \toprule
\end{tabular}%}
%\end{adjustbox}
\caption{Number of sentences for different NER datasets}\label{tab:NERdata}
\end{table}

==> Tables/other_information/commonsense.tex <==
\begin{table*}[!ht]
\small 
\centering
\begin{adjustbox}
\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{3cm}p{2cm}p{7cm}}
%p{3cm}p{3cm}p{3cm}p{3cm}p{3cm}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Sent}} 
\\ \toprule
                        %& $0.625$\% & $0.613$\% \\
 \multirow{}{}\textbf{X-CSQA}  & \textbf{question:}  &james alipenda nyota. Nyikani, waliangaza nini? \\
                                  & \textbf{choices:}  &"A", "text": "nafasi ya nje"\\
                                  &  &"B", "text": "obiti",  \\
                                  &  &"C", "text": "ulimwengu",\\
                                  &  &"D", "text": "anga la usiku", \\
                                  &  &"E", "text": "ardhi",  \\
                                  & \textbf{answer key:} & "D" \\
                                  \hline
 \multirow{}{}\textbf{X-CODAH}   & \textbf{question-tag:} & "o"    \\ 
                                 & \textbf{choices:}   & "A", "text": "Mtu anaruka ndege ya sura ya joka. Yeye hufanya kazi kwa laini ili kufanya joka lifanye matanzi marefu kupitia hewani.",   \\
                                  & & "B", "text": "Mtu anaruka ndege ya sura ya joka. Anaweka haradali kwenye mbwa moto na kumkabidhi mteja.",    \\
                                  & &"C", "text": "Mtu anaruka ndege ya sura ya joka. Anamaliza kukata na kuanza kupalilia bustani.",     \\
                                  & & "D", "text": "Mtu anaruka ndege ya sura ya joka. Yeye huchota upanga wake na kuanza kushambulia joka." \\
                                  & \textbf{answerKey:} & "A"      \\
 \toprule
\end{tabular}}
\end{adjustbox}
\caption{Examples from X-CSQA and X-CODAH}\label{tab:commonsense}
\end{table*}


==> Tables/other_information/morph_segmentation.tex <==
\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Tokens}}
\\
 \toprule
% <af>, <nso> <ss> <st> <tn> <ts> <ve> <zu>
~   
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/320}{Zulu}  &$36,092$ \\%& $0.616$\% & $0.605$\% \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Sesotho}  &$57,904$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Siswati}  &$34,406$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/363}{Xitsonga}  &$57,586$  \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/329}{Sepedi}  &$57,987$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/300?show=full}{Afrikaans}  &$55,537$ \\
                                   & \href{https://repo.sadilar.org/handle/20.500.12185/342}{Setswana}  &$57,526$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/356}{Tshivenda}  &$55,069$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/307}{Isindebele} & $33,400$\\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/313}{Xhosa} & $36,537$ \\
 \toprule
\end{tabular}%}


%\end{adjustbox}
\caption{Number of tokens for the morphological segmentation data for each language.}\label{tab:morphdata}
\end{table}


==> Tables/other_information/news.tex <==

\begin{table}[!ht]
\small
\centering
\begin{tabular}{p{2cm}p{4cm}} 
\toprule
\thead{\textbf{Counts}} & \thead{\textbf{Dataset}}  \\ \toprule
$171,090$ & \href{https://github.com/IsraelAbebe/An-Amharic-News-Text-classification-Dataset/blob/main/data/Amharic\%20News\%20Dataset.zip}{Amharic-news-classification}  \\ \hline
$21,270$ & \href{https://github.com/Andrews2017/KINNEWS-and-KIRNEWS-Corpus}{KINNEWS Corpus} \\ \hline
$4,614$ & \href{https://github.com/Andrews2017/KINNEWS-and-KIRNEWS-Corpus}{KIRNEWS Corpus}\\ \hline
$145,033$ &  \href{https://zenodo.org/record/4300294#.YcQSQGDMJyz}{Swahili: News Classification Dataset}\\ \hline
$185,980$ &  \href{https://zenodo.org/record/4300294#.YcQSQGDMJyz}{Swahili: News Classification Dataset version 2}\\ \hline
$8,137$ &  \href{https://github.com/uds-lsv/transfer-distant-transformer-african/tree/master/data}{Hausa Topic Classification}\\ \hline
$4,757$ & \href{https://github.com/uds-lsv/transfer-distant-transformer-african/tree/master/data}{Y{o}r\`{u}b\'{a} Topic Classification}\\ \hline
 \end{tabular}
 \caption{Statistics information for news classification datasets} \label{tab:news_classification}
 \end{table}

==> Tables/other_information/phrasechunks.tex <==

\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Tokens}}
\\
 \toprule
% <af>, <nso> <ss> <st> <tn> <ts> <ve> <zu>
~   
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/320}{Zulu}  &$16,262$ \\%& $0.616$\% & $0.605$\% \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Sesotho}  &$15,798$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Siswati}  &$16,008$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/363}{Xitsonga}  &$15,948$  \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/329}{Sepedi}  &$15,640$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/300?show=full}{Afrikaans}  &$15,660$ \\
                                   & \href{https://repo.sadilar.org/handle/20.500.12185/342}{Setswana}  &$15,774$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/356}{Tshivenda}  &$15,598$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/307}{Isindebele} & $15,945$\\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/313}{Xhosa} & $14,010$ \\
 \toprule
\end{tabular}%}
%\end{adjustbox}
\caption{Number of tokens for the phrase chunks dataset for each language.}\label{tab:phrasedata}
\end{table}

==> Tables/other_information/pos.tex <==
\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}  %{lcrr}
 \toprule
\multicolumn{}{}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{}{}{\textbf{#Tokens}} % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
\\
 \toprule
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{Masakhane-Wazobia }}   & \href{https://github.com/masakhane-io/masakhane-wazobia-dataset/blob/master/Data/Urhobo_words/Urhobo.csv}{Urhobo}  &$2,019$ \\ \\
                                  \hline
                                  
\multirow{}{} {\textbf{IgboNLP}}   & \href{https://github.com/Iykeln/IgboNLP/blob/master/IgboTaggedCorpus/}{Igbo}  &$2,019$ \\
                                  \hline
                
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/293}{Afrikaans}  &$58,945$   \\ 
                                 & \href{https://repo.sadilar.org/handle/20.500.12185/302}{Isindebele}  &$42,332$   \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/309}{Isixhosa}  &$42,062$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/315}{Isizulu}  &$41,715$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/325?show=full}{Sepedi}  &$62,842$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/332}{Sesotho}  &$62,926$     \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/337}{Sestwana}  &$62,843$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/344}{Siswati}  &$39,487$     \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/353}{Tshivenda}  &$59,815$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/359}{Xitsonga}  &$62,956$    \\\hline
 \toprule
\end{tabular}%}
%\end{adjustbox}
\caption{Number of tokens used for POS tagging for each language.}\label{tab:pos}
\end{table}

==> Tables/other_information/sentiment.tex <==
\begin{table}[!ht]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule 
\multicolumn{}{}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{}{}{\textbf{#Sent}}  % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
\\
 \toprule
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{Bambara}}   & \textbf{Bambara}  &$3,046$  \\
                               \hline
 \multirow{}{} {\textbf{Yoruba}}   & \textbf{Yoruba}  &$3,006$\\ \hline
 \multirow{}{} {\textbf{N.Pidgin}}   & \textbf{N.Pidgin}  &$14,001$\\ 
                                 & \textbf{N.Pidgin}  &$11,760$ \\
          
 \toprule
\end{tabular}
\caption{Number of sentences for sentiment analysis data.}\label{tab:sentiment}
\end{table}


==> downstream_tasks.tex <==
\section{Tasks and Datasets}\label{sec:downstream}
We test the utility of our LMs on $5$ token level and $5$ sentence level downstream tasks. We use a combination of existing datasets and create new ones too.

\subsection{Token Level}

\textbf{Named Entity Recognition (NER)}
We evaluate our models on NER datasets across multiple languages. We used MasakhaneNER data \cite{ifeoluwa2021masakhaner}, WikiAnn \cite{pan2017cross, rahimi-etal-2019-massively}, Yoruba-Twi NER data \cite{alabi2020massive}, Distance Supervision NER (DS NER) Data \cite{hedderich-etal-2020-transfer} and multiple NER data from \href{https://repo.sadilar.org/handle/20.500.12185/7}{SADiLaR}. Data from SADiLaR covered $10$ indigenous South African languages and is annotated for person, organisation, location and miscellaneous named entities. Where miscellaneous named entities refer to all rigid designators that do not fall into one of the other categories, including temporal expressions (dates and times), URLs, numerical expressions, publications, names of languages, nationalities, among others. We provide detailed statistics of the datasets in Table \ref{tab:NERdata}. 

\subsection{Morphological Segmentation}
We evaluate our models on morphological segmentation data for $10$ South African languages. The data identifies the morphemes of each token particularly those for morphologically complex words. The data is annotated across $20$ main categories including: nouns, verbs and auxiliary verbs, adjectives, adverbs, subject and object concords, demonstratives, pronouns, copulatives, particles and prepositions, secondary morphemes, ideophones, possessive concords, interjections, conjunctions, interrogatives, abbreviations, demonstrative copulatives, enumeratives, and past tense markers. Each of these categories are then labelled as root, stem, suffix, prefix, or any other appropriate morphological label. We provide some statistical information about the dataset in Table \ref{tab:morphdata}.

\subsection{Phrase Chunks}
We evaluate our models on phrase chunks datasets for $10$ indigenous languages of South Africa. We provide a table showing the statistics of the datasets in Table \ref{tab:phrasedata}. The data has annotations for noun, verb, adjective, adverbial, and prepositional phrase chunks. Words not belonging to these phrase types are labelled with \textit{o}. 

\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Tokens}}
\\
 \toprule
% <af>, <nso> <ss> <st> <tn> <ts> <ve> <zu>
~   
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/320}{Zulu}  &$16,262$ \\%& $0.616$\% & $0.605$\% \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Sesotho}  &$15,798$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Siswati}  &$16,008$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/363}{Xitsonga}  &$15,948$  \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/329}{Sepedi}  &$15,640$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/300?show=full}{Afrikaans}  &$15,660$ \\
                                   & \href{https://repo.sadilar.org/handle/20.500.12185/342}{Setswana}  &$15,774$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/356}{Tshivenda}  &$15,598$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/307}{Isindebele} & $15,945$\\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/313}{Xhosa} & $14,010$ \\
 \toprule
\end{tabular}%}


%\end{adjustbox}
\caption{Number of tokens for the phrase chunks dataset for each language.}\label{tab:phrasedata}
\end{table}


%subsection{Machine Translation}
%We evaluate our models on various MT datasets and benchmarks. 

%\begin{table}[!ht]
%\small 
%\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
%\begin{tabular}{lcrr}
% \toprule
%\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Sent}}  % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
%\\
% \toprule
%\multirow{2}{*} {\textbf{Masakhane-NER}}  & \textbf{Hausa} & $11,154$\\ %& $0.453$\% & $0.448$\%\\
%                                  & \textbf{Igbo} & $11,154$ \\
%                                  & \textbf{Yoruba} & $11,154$\\
%                                  & \textbf{Amharic} & $11,154$ \\
%                                  & \textbf{Kinyarwanda} & $11,154$  \\
%                                  & \textbf{Luo} & $11,154$ \\
%                                  & \textbf{Luganda} & $11,154$  \\
%                                  & \textbf{Naija Pidgin} & $11,154$ \\
%                                  & \textbf{Setswana} & $11,154$ \\
%                                  & \textbf{Shona} & $11,154$ \\
%                                  & \textbf{Swahili} & $11,154$  \\
%                                  & \textbf{Wolof} & $11,154$ \\
                        %& $0.44$\%  &$0.419$\%  \\
%                        \hline
%\multirow{2}{*} {\textbf{WikiAnn}}   & \textbf{Yoruba}  &$31,086$  \\%& $0.616$\% & $0.605$\% \\
%                                  & \textbf{Akan}  &$31,086$   \\
%                                  & \textbf{Twi}  &$31,086$   \\
%                                  & \textbf{Swahili}  &$31,086$    \\
%                                  & \textbf{Amharic}  &$31,086$   \\
%                                  & \textbf{Kinyarwanda}  &$31,086$   \\
%                                  \hline
                        %& $0.625$\% & $0.613$\% \\
%\multirow{2}{*} {\textbf{NCHLT}}   & \textbf{Zulu}  &$31,086$ \\%& $0.616$\% & $0.605$\% \\
%                                  & \textbf{Xhosa}  &$31,086$   \\
%                                  & \textbf{Sesotho}  &$31,086$  \\
%%                                  & \textbf{Siswati}  &$31,086$  \\
%                                  & \textbf{Xitsonga}  &$31,086$ \\
%                                  & \textbf{Sepedi}  &$31,086$  \\
%                                  & \textbf{Ndebele}  &$31,086$  \\
%                                  & \textbf{Afrikaans}  &$31,086$ \\
%                                   & \textbf{Setswana}  &$31,086$  \\
%                                    & \textbf{Tshivenda}  &$31,086$ \\
%                                  \hline
% \toprule
%\end{tabular}%}
%\end{adjustbox}
%\caption{Number of sentences and words for the training data used for each language pair.}\label{tab:data}
%\end{table}

\subsection{Lemmatization}
We test our models on lemmatization dataset for $10$ South African Languages. We provide the statistical information for the dataset in Table \ref{tab:lemmadata}.

\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule 
\multicolumn{}{}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{}{}{\textbf{#Tokens}}
\\ 
 \toprule
% <af>, <nso> <ss> <st> <tn> <ts> <ve> <zu>
~   
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/320}{Zulu}  &$33,752$ \\%& $0.616$\% & $0.605$\% \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Sesotho}  &$57,703$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/335}{Siswati}  &$34,394$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/363}{Xitsonga}  &$55,463$  \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/329}{Sepedi}  &$57,780$ \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/300?show=full}{Afrikaans}  &$55,407$ \\
                                   & \href{https://repo.sadilar.org/handle/20.500.12185/342}{Setswana}  &$57,421$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/356}{Tshivenda}  &$52,834$  \\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/307}{Isindebele} & $36,682$\\
                                    & \href{https://repo.sadilar.org/handle/20.500.12185/313}{Xhosa} & $36,428$ \\
 \toprule
\end{tabular}%}


%\end{adjustbox}
\caption{Number of tokens for the phrase chunks dataset for each language.}\label{tab:lemmadata}
\end{table}

\subsection{Part of Speech Tagging}
We test our models on POS tagging datasets for various languages. We use data from Masakhane-Wazobia, IgboNLP \cite{10.1145/3146387, 10.1145/3314942} and SADiLaR. The dataset from M.W provides POS tags for words in isolation. In Table \ref{tab:pos}, we provide the statistical details for each dataset we use.

\begin{table}[!h]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}  %{lcrr}
 \toprule
\multicolumn{}{}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{}{}{\textbf{#Tokens}} % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
\\
 \toprule
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{Masakhane-Wazobia }}   & \href{https://github.com/masakhane-io/masakhane-wazobia-dataset/blob/master/Data/Urhobo_words/Urhobo.csv}{Urhobo}  &$2,019$ \\ \\
                                  \hline
                                  
\multirow{}{} {\textbf{IgboNLP}}   & \href{https://github.com/Iykeln/IgboNLP/blob/master/IgboTaggedCorpus/}{Igbo}  &$2,019$ \\
                                  \hline
                
\multirow{}{} {\textbf{NCHLT}}   & \href{https://repo.sadilar.org/handle/20.500.12185/293}{Afrikaans}  &$58,945$   \\ 
                                 & \href{https://repo.sadilar.org/handle/20.500.12185/302}{Isindebele}  &$42,332$   \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/309}{Isixhosa}  &$42,062$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/315}{Isizulu}  &$41,715$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/325?show=full}{Sepedi}  &$62,842$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/332}{Sesotho}  &$62,926$     \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/337}{Sestwana}  &$62,843$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/344}{Siswati}  &$39,487$     \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/353}{Tshivenda}  &$59,815$    \\
                                  & \href{https://repo.sadilar.org/handle/20.500.12185/359}{Xitsonga}  &$62,956$    \\\hline
 \toprule
\end{tabular}%}
%\end{adjustbox}
\caption{Number of tokens used for POS tagging for each language.}\label{tab:pos}
\end{table}

\subsection{Sentiment Analysis}
We finetuned our model on three sentiment analysis datasets available for Bambara \cite{diallo2021bambara}, Yoruba \cite{shode_africanlp}, and the Nigerian Pidgin \cite{oyewusi2020semantic} respectively. We show some details of these datasets in Table \ref{tab:sentiment}.
\begin{table}[!ht]
\small 
\centering
%\begin{adjustbox}{width=6cm}
%\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{2cm}p{2cm} p{1cm}}
 \toprule 
\multicolumn{}{}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{}{}{\textbf{#Sent}}  % & %\multicolumn{1}{c}{\textbf{Untok TTR}} & \multicolumn{1}{c}{\textbf{Tok TTR}}
\\
 \toprule
                        %& $0.625$\% & $0.613$\% \\
\multirow{}{} {\textbf{Bambara}}   & \textbf{Bambara}  &$3,046$  \\
                               \hline
 \multirow{}{} {\textbf{Yoruba}}   & \textbf{Yoruba}  &$3,006$\\ \hline
 \multirow{}{} {\textbf{N.Pidgin}}   & \textbf{N.Pidgin}  &$14,001$\\ 
                                 & \textbf{N.Pidgin}  &$11,760$ \\
          
 \toprule
\end{tabular}
\caption{Number of sentences for sentiment analysis data.}\label{tab:sentiment}
\end{table}


\subsection{News classification}
We used news classification datasets for Amharic \cite{azime2021amharic}, Kinyarwanda \cite{niyongabo-etal-2020-kinnews}, Kirundi \cite{niyongabo-etal-2020-kinnews}, and Swahili \cite{davis_david_2020_4300294, davis_david_2020_5514203}. The Amharic dataset contains 6 classes - news, sport, politics, international news, business, and entertainment. The Swahili dataset also has $6$ categories including local news, international, finance, health, sports, and entertainment. The datasets for Kinyarwanda and Kirundi have $14$ and $12$ categories each. Each category is labelled with a number starting from $1$ through $14$ for Kinyarwanda and $1$ through $12$ for Kirundi \cite{niyongabo-etal-2020-kinnews}. The categories are $1$ politics, $2$ sports, $3$ economy, $4$ health, $5$ entertainment, $6$ history, $7$ technology, $8$ tourism, $9$ culture, $10$ fashion $11$ religion $12$ environment, $13$ education, and $14$ relationship. Table \ref{tab:news_classification} contains statistics information of the datasets we use. We also include here topic classification datasets for for Y{o}r\`{u}b\'{a} and Hausa \cite{hedderich-etal-2020-transfer}.  The Y{o}r\`{u}b\'{a} and Hausa datasets contains news titles collected from VOA Hausa and BBC Y{o}r\`{u}b\'{a} news sites. The Y{o}r\`{u}b\'{a} dataset has $7$ topics - Nigeria, Africa, world, entertainment, health, sports, and politics, while the Hausa dataset is categorized into $5$ topics - Nigeria, Africa, world, health, and politics. 

\begin{table}[!ht]
\small
\centering
\begin{tabular}{p{2cm}p{4cm}} 
\toprule
\thead{\textbf{Counts}} & \thead{\textbf{Dataset}}  \\ \toprule
$171,090$ & \href{https://github.com/IsraelAbebe/An-Amharic-News-Text-classification-Dataset/blob/main/data/Amharic\%20News\%20Dataset.zip}{Amharic-news-classification}  \\ \hline
$21,270$ & \href{https://github.com/Andrews2017/KINNEWS-and-KIRNEWS-Corpus}{KINNEWS Corpus} \\ \hline
$4,614$ & \href{https://github.com/Andrews2017/KINNEWS-and-KIRNEWS-Corpus}{KIRNEWS Corpus}\\ \hline
$145,033$ &  \href{https://zenodo.org/record/4300294#.YcQSQGDMJyz}{Swahili: News Classification Dataset}\\ \hline
$185,980$ &  \href{https://zenodo.org/record/4300294#.YcQSQGDMJyz}{Swahili: News Classification Dataset version 2}\\ \hline
$8,137$ &  \href{https://github.com/uds-lsv/transfer-distant-transformer-african/tree/master/data}{Hausa Topic Classification}\\ \hline
$4,757$ & \href{https://github.com/uds-lsv/transfer-distant-transformer-african/tree/master/data}{Y{o}r\`{u}b\'{a} Topic Classification}\\ \hline
 \end{tabular}
 \caption{Statistics information for news classification datasets} \label{tab:news_classification}
 \end{table}

\subsection{CommonSense Reasoning}
We use \href{https://inklab.usc.edu/XCSR/xcsr_datasets?msclkid=90d70283b60111ecb0f6bcf7104eb3c3}{X-CSQA} and \href{https://inklab.usc.edu/XCSR/xcsr_datasets?msclkid=90d70283b60111ecb0f6bcf7104eb3c3}{X-CODAH} datasets \cite{lin-etal-2021-xcsr, Talmor2019commonsenseqaaq, Chen2019CODAHAA}. X-CSQA is a multiple-choice QA task that requires general information about the world, otherwise referred to as commonsense knowledge. According to \cite{https://doi.org/10.48550/arxiv.2204.02311} commonsense reasoning tasks not simply factual question answering but require the combination of multiple logical inferences about the world. The datasets are multilingual, however since we focus on African languages, we use the data for Swahili which is the only African language represented in the datasets. X-CSQA contains $1,000$ examples for development and $1,074$ examples for testing. X-CODAH on the other hand has $300$ development examples and $1,000$ testing examples. X-CSQA dataset format includes a question, $5$ answer options, and an answer key. X-CODAH uses a question tag with $6$ options: i, n, p, r, q, o - representing idioms, negation, polysemy, reference, quantitative and other respectively. It has $4$ answer options and an answer key. We show examples for both dataset in Table~\ref{tab:commonsense}.

\begin{table*}[!ht]
\small 
\centering
\begin{adjustbox}
\renewcommand{\arraystretch}{1.5}{
\begin{tabular}{p{3cm}p{2cm}p{7cm}}
%p{3cm}p{3cm}p{3cm}p{3cm}p{3cm}
 \toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Lang}} & \multicolumn{1}{c}{\textbf{#Sent}} 
\\ \toprule
                        %& $0.625$\% & $0.613$\% \\
 \multirow{}{}\textbf{X-CSQA}  & \textbf{question:}  &james alipenda nyota. Nyikani, waliangaza nini? \\
                                  & \textbf{choices:}  &"A", "text": "nafasi ya nje"\\
                                  &  &"B", "text": "obiti",  \\
                                  &  &"C", "text": "ulimwengu",\\
                                  &  &"D", "text": "anga la usiku", \\
                                  &  &"E", "text": "ardhi",  \\
                                  & \textbf{answer key:} & "D" \\
                                  \hline
 \multirow{}{}\textbf{X-CODAH}   & \textbf{question-tag:} & "o"    \\ 
                                 & \textbf{choices:}   & "A", "text": "Mtu anaruka ndege ya sura ya joka. Yeye hufanya kazi kwa laini ili kufanya joka lifanye matanzi marefu kupitia hewani.",   \\
                                  & & "B", "text": "Mtu anaruka ndege ya sura ya joka. Anaweka haradali kwenye mbwa moto na kumkabidhi mteja.",    \\
                                  & &"C", "text": "Mtu anaruka ndege ya sura ya joka. Anamaliza kukata na kuanza kupalilia bustani.",     \\
                                  & & "D", "text": "Mtu anaruka ndege ya sura ya joka. Yeye huchota upanga wake na kuanza kushambulia joka." \\
                                  & \textbf{answerKey:} & "A"      \\
 \toprule
\end{tabular}}
\end{adjustbox}
\caption{Examples from X-CSQA and X-CODAH}\label{tab:commonsense}
\end{table*}

\subsection{Question Answering}
We use \href{https://github.com/google-research-datasets/tydiqa}{TYDIA} question answering dataset \cite{clark-etal-2020-tydi}. The dataset has a primary task and a gold passage task. The primary task has two tasks, a passage selection task and a minimal answer span task. For the passage selection task, a list of passages is given and the required response is either the index of the passage where the answer to the question is or null, if no answer exists in the passage. The minimal answer span task on the other hand gives a full article and the expected answer is either the start and end byte indices of the minimal span that answers the question, yes or no response, or null, if no minimal answer exist. For the gold passage task, a correct answer is predicted from a passage containing one answer. This is similar to existing reading comprehension. We use the Kiswahili dataset alone, since it is the only African language in the dataset. It contains $17,613$ training, $2,288$, development, and $2,278$ test examples. 

\subsection{Word Similarity}
We use WordSim and Simlex datasets for Sepedi and Setswana \cite{Makgatho_2021} and WordSim dataset for Twi and Y{o}r\`{u}b\'{a} \cite{alabi-etal-2020-massive}. These datasets are translations of the original WordSim \cite{Finkelstein2001PlacingSI} and Simlex \cite{HillRK15}. The Y{o}r\`{u}b\'{a} set was translated by $3$ native speakers and is composed of $446$ translations. $348$ of which are single-word translations, $61$ are transliterations, and $98$ are short phrases. The Twi translations consist of $298$ single word translations and $4$ transliterations.

We show the statistics for the datasets in Table~\ref{tab:wordsim}.

\begin{table}[H]
\centering
\begin{tabular}{p{3cm}p{2cm}} 
\toprule

\thead{\textbf{Dataset}} & \thead{\textbf{Size}}  \\ \toprule
 \href{https://zenodo.org/record/5673974/files/SimLex-999-orig\%20-\%20Sepedi.xlsx?download=1}{simlex Sepedi} & $1,000$ \\ \hline
 \href{https://zenodo.org/record/5673974/files/SimLex-999-orig\%20-\%20Setswana.xlsx?download=1}{simlex Setswana} & $1,000$ \\ \hline \href{https://github.com/ajesujoba/YorubaTwi-Embedding/blob/master/Yoruba/wordSim353_yo.csv}{wordSim Y{o}r\`{u}b\'{a}} & $354$\\ \hline
 \href{https://zenodo.org/record/5673974/files/wordsim353_orig\%20-\%20Setswana.xlsx?download=1}{wordSim Setswana} & $354$\\ \hline  \href{https://github.com/ajesujoba/YorubaTwi-Embedding/blob/master/Twi/wordsim_tw.csv}{wordSim Twi} & $275$\\ \hline
 \href{ https://zenodo.org/record/5673974/files/wordsim353_orig\%20-\%20Sepedi.xlsx?download=1}{wordSim Sepedi} & $1000$\\ \hline

 \end{tabular}
 \caption{Statistics for Word Similarity Datasets} \label{tab:wordsim}
 \end{table}
 
 \subsection{Language Identification}
Language identification (LID) focuses on identifying the human language a piece of text or speech segment belongs to, making automatic LID an important first step in processing human language appropriately~\cite{tjandraetal2021improved, thara_etal_2021}. We use datasets from AfroLID \cite{} for this task. AfroLID data is a multi-genre, multi-script dataset for $517$ African languages. We compare the performance of AfroLID data on our models with performance on AfroLID tool. We show results in Table XXX 

==> families_eval.tex <==
\section{Typology Evaluation}\label{sec:families}
This analysis is motivated by the competitive results we report in zero-shot settings for XLMR, mBERT, Afro-XLMR, and AfriBERTa on certain languages. Specifically, we wanted to investigate the influence of linguistic similarity between languages used in training and those used in zero-shot settings. To do this, we measure the Jaccard similarity between the African languages used in training each model and the languages used in zero-shot settings. This analysis thus involves similarity measures between $30$ languages, which is a superset of all languages used for training and zero-shot settings on all models.\footnote{We will add results of this analysis to the next version of this paper.}

%We evaluate the performance of our model on each task gleaning insights from the family relationship in model performance. Specifically, we wanted the investigate the role of mutual intelligibility or linguistic similarity of model performance as well as zero shot learning. Overall, we find that although many of these languages are mutually intelligible, the similarity scores are neligible, giving the impression that the mutual intelligibility is not evident in the orthography of these languages. 

% \noindent\textbf{Afro-Asiatic.} Our Afroasiatic family consist of Amharic, Hausa,  Oromo, Somali, and Tigrinya. Figure~\ref{fig:afroasiatic} shows the relationship between these languages.
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/afro-asiatic.png}
% \caption{\small Afro-Asiatic languages in \ourmodel. Amharic (amh), Hausa (hau), Oromo (gaz), Somali (som) and Tigrinya (tir) are presented in red circles.}\label{fig:afroasiatic} 
% \end{figure}

% \noindent\textbf{Austronesean.} Malagasy is the only language in the Austronesean family. We show the family information in Figure~\ref{fig:austronesean} 
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/austronesean.png}
% \caption{\small Austroneasean language family consisting of Malagasy (mlg).}\label{fig:austronesean} 
% \end{figure}

% \noindent\textbf{Creole}
% Nigerian Pidgin is an English-based creole in our downstream task. It is the only creole represented in our downstream task. We show the family information in Figure~\ref{fig:creole} 
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/creole.png}
% \caption{\small Creole language family consisting of Nigerian Pidgin (pcm).}\label{fig:creole} 
% \end{figure}

% \noindent\textbf{Indo-European}
% Afrikaans is the only Indo-European language of Africa. Figure~\ref{fig:indoeuropean} shows the genetic information.
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/indo-european.png}
% \caption{\small Indo-European language family consisting of Afrikaans (afr).}\label{fig:indoeuropean} 
% \end{figure}

% \noindent\textbf{Niger Congo}
% Our Niger Congo family includes Bambara, Chichewa, Igbo, isiXhosa, isiZulu, Kirundi, Kinyawanda, Luganda, Luo, Ndebele, Sepedi, Sesotho, Siswati, Tswana, Tsonga, Shona, Swahili, Venda, Wolof, and Yoruba. Relationship between these languages is captured in Figure~\ref{fig:nigercongo} 
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/niger_congo.png}
% \caption{\small Niger Congo language family.}\label{fig:nigercongo} 
% \end{figure}

% \noindent\textbf{Nilo Saharan}
% Luo is the only Nilo Saharan language in our benchmark. The genetic information for this language is shown in Figure~\ref{fig:nilosaharan} 
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/nilo-saharan.png}
% \caption{\small Nilo Saharan language family with Luo (luo)}\label{fig:nilosaharan} 
% \end{figure}

\input{Tables/jacc_sim.tex}
We provide jaccard similarity results for the superset of languages represented in our benchmarkin Table \ref{tab:jacc_sim}.



==> mlm.tex <==
\section{Language Models}\label{sec:motivation}
\input{Tables/resources}
\input{Tables/encoder-only-models}

\subsection{With African Languages}
A couple of LMs support some African languages. We provide an overview below:

\noindent{\textbf{mBERT}} \cite{devlin-etal-2019-bert} is a multilingual variant of BERT trained on $104$ languages. 

\noindent{\textbf{AfriBERTa}} \cite{ogueji-etal-2021-small} is a language model focused on 11 African languages including: Afaan Oromoo, Amharic, Gahuza (a code-mixed language of Kinyarwanda and Kirundi), Hausa, Igbo, Nigerian Pidgin, Somali, Swahili, Tigrinya and Yoruba. The pretraining corpus for this model is small with only $108.8$ million tokens, when compared to a typical language model. AfriBERTa is trained using a transformer with the standard masked language modelling objective. AfriBERTa model uses $6$ attention heads, $768$ hidden units, $3072$ feed forward dimensions and a maximum length of $512$ for the $3$ configurations of the model. The parameter sizes are $97$, $111$, and $126$ million respectively. 

\noindent{\textbf{KINYaBERT}} \cite{nzeyimana-niyongabo-rubungo-2022-kinyabert} uses a two-tier BERT architecture that comprises of a morphological analyzer and explicitly represents morphological information for Kinyawanda - a morphologically rich African language. They show that KINYaBERT achieves better convergence, gets better accuracy, and robust results on multiple downstream tasks. They further compare the performance 

%Mention Quality of dataset is good, diverse, multilingual; population statistics. 

%Multitask for langid - 

%W of Devlin et al. (2019) without next sentence prediction. This is also the same approach used in XLM-R (Conneau et al., 2020). We pretrain on text data containing all languages, sampling batches from different languages. We sample languages such that our model does not see the same language over several consecutive batches.

\noindent{\textbf{Afro-XLM-R}} \cite{https://doi.org/10.48550/arxiv.2204.06487} uses language adaptation on the 17 most-resourced African languages and three other high-resource foreign language widely used in Africa – English, French, and Arabic – simultaneously to provide a single model for cross-lingual transfer learning for African languages. 

\noindent{\textbf{XLM-R}} \cite{conneau-etal-2020-unsupervised} uses a transformer based architecture and obtains state-of-the-art performance on cross-lingual classification, sequence labeling, and question answering on $100$ languages. The training procedure uses a masked language model similar to that for XLM although some changes that improve performance are introduced. The model uses a multilingual objective with monolingual data and the model learns to predict the masked tokens as the streams of text are sampled from each language. They show that scaling the number of languages for a fixed model capacity leads to better cross-lingual performance on low resource languages. They however show that performance degrades after a while, although this can be alleviated by increasing model capacity. To ensure that their model deals better with code switching, they do not use language embeddings. 

\subsection{Without African Languages}
% \noindent{\textbf{BERT}}
% BERT \cite{devlin-etal-2019-bert} is trained on unlabeled data over two pre-training tasks: masked LM and next sentence prediction. For fine-tuning, the BERT model is first initialized with the pre-trained parameters, and all of the parameters are fine-tuned using labeled data from the downstream tasks. Each downstream task has a separate fine-tuned model, although they are initialized with the same pre-trained parameters. BERT uses a unified architecture across different tasks with minimal distinctions between the pre-trained model and the downstream tasks. The input representation referred to as a \textit{Sentence} is carefully crafted to handle a variety of tasks. It accommodates an arbitrary sequence of contiguous texts so that a single BERT sentence can be one or two traditional sentences packed together.
% BERT’s architecture is a multi-layer bidirectional Transformer encoder with $12$ layers, $768$ hidden layers, $12$ attention heads and $110M$ parameters for the base model and $24$ layers, $1,024$ hidden layers, $16$ attention heads and $340M$ parameters for the large model. 

% \noindent{\textbf{Roberta}}
% Roberta \cite{liu2019roberta} improves on the BERT model by carefully training and tuning key hyperparameters and training data size. The BERT model is re-implemented with the original optimization hyperparameters, although the peak learning rate and number of warmup steps are tuned separately for each setting. They show that training is sensitive to the Adam epsilon term and in some cases better performance or improved stability was obtained
% after tuning it. They also set $β2$ to $0.98$ to improve stability when training with large batch sizes. They also show significant gains in downstream task performance, with longer training of up to 500K steps and with more data. They train with token sizes not greater than $512$ and unlike the original BERT implementation which randomly injects short sentences, they train only with full length sequences for the first $90\%$ of updates.

\noindent{\textbf{Electra}}
\cite{Clark2020ELECTRA, chi2021xlme} trains two neural networks, a generator \textbf{G} and a discriminator \textbf{D}. Each network consists of an encoder that maps a sequence of input tokens into a sequence of contextualized vector representations. The generator on one hand is a small BERT model trained with the masked language modeling task. The discriminator on the other learns to predict the original identities of the masked-out tokens, that is to distinguish tokens in the data from tokens that have been replaced by generator samples. Although Electra's training objective is similar to that of a generative adversarial network (GAN) \cite{NIPS2014_5ca3e9b1}, it differs in a number of ways. First, the generator generates real tokens rather than fakes as in GANs. Second, the generator uses a maximum likelihood rather than an adversarial training. Finally, the generator does not use a noise vector which is a typical input feature for GANs. The model architecture and most hyperparameters are the same as BERT’s. For Fine-tuning on GLUE, a simple linear classifier is added on top of ELECTRA while an answerability classifier is added on top of Electra for SQuAD. They also report the median of 10 fine-tuning runs on the evaluation datasets. Electra greatly reduces the computation cost of cross-lingual pretraining and 
encourages better cross-lingual transferability \cite{chi2021xlme}.



==> pretraining-data.tex <==
\section{PreTraining Data}\label{sec:pretraining}
Our model is trained using a multi-domain language identification corpus we develop. This corpus contains texts $5$ different domains including: religious, news, government documents, health, and internet crawls. We collect $70.7M$ sentences for $517$ languages across $14$ language families and randomly select $5,000$, $50$, and $100$ sentences for train, development, and test respectively for each language. In all, the langid training data comprises of $2,496,980$ for training, $25,700$ for development, and $51,400$ for test.  We provide a description of each of these datasets.

\subsection{Religious Domain}
Our religious data is taken from online bibles, qurans, and data crawled from the Jehovah's Witness website. We also include other religious texts like those from the book of mormon. 
%provide details of the data from this domain. 
% \subsubsection{Bibles}
% We crawled bibles from \hyperlink{https://www.biblegateway.com}{Bible Gateway} and \hyperlink{https://www.bible.com/en-GB/languages}{Youversion} for $498$ languages. The bible is divided into the old testament and the new testament. The old testament has $39$ books and the new testament has $27$ books. The books are written in chapters with $1,189$ chapters in all - $929$ in the old testament and $260$ chapters in the new testament. These chapters are further divided into verses, There are $23,145$ verses in the Old Testament and $7,957$ verses in the New Testament. This gives a total of $31,102$ verses although the number of verses may differ across languages.

% \subsubsection{Quran}


% \subsubsection{Jehovah's Witness}
% We crawled text from \hyperlink{https://www.jw.org/en/}{Jehovah's Witness} website for $146$ African languages. We collected data for 

% \subsubsection{Other Religious Texts}
% This contains religious articles for 

\subsection{News Domain}
We collect data from online newspapers, and international news sites such as Voice of America, BBC, Global voices and DW news sites. We also collect local newspapers across $27$ languages. 

% Detailed description are available in Table xx.
% \subsubsection{Voice of America}
% We crawled data from the \hyperlink{https://www.voanews.com/navigation/allsites}{Voice of America} website for \hyperlink{https://www.voaafaanoromoo.com/}{Afaan}, \hyperlink{https://amharic.voanews.com/}{Amharic}, \hyperlink{https://www.voabambara.com/}{Bambara}, \hyperlink{https://www.voahausa.com/}{Hausa}, \hyperlink{https://www.radiyoyacuvoa.com/}{Kinyawanda}, \hyperlink{https://www.voalingala.com/}{Lingala}, \hyperlink{https://www.voandebele.com/}{Ndebele}, \hyperlink{https://www.voashona.com/}{Shona}, \hyperlink{https://www.voasomali.com/}{Somali}, \hyperlink{https://www.voaswahili.com/}{Swahili}, and \hyperlink{https://tigrigna.voanews.com/}{Tigrigna}
% \subsubsection{BBC}
% We crawled data from \hyperlink{https://www.bbc.co.uk/ws/languages}{BBC} for \hyperlink{https://www.bbc.com/afaanoromoo}{Afaan}, \hyperlink{https://www.bbc.com/amharic}{Amharic}, \hyperlink{https://www.bbc.com/hausa}{Hausa}, \hyperlink{https://www.bbc.com/igbo}{Igbo}, \hyperlink{https://www.bbc.com/gahuza}{Kinyarwanda}, \hyperlink{https://www.bbc.com/pidgin}{Nigerian Pidgin}, \hyperlink{https://www.bbc.com/somali}{Somali}, \hyperlink{https://www.bbc.com/swahili}{Swahili}, \hyperlink{https://www.bbc.com/tigrinya}{Tigrinya}, and \hyperlink{https://www.bbc.com/yoruba}{Yoruba}.

% \subsubsection{Global Voices}
% We collected news text from the \hyperlink{}{Global Voices} website for the following languages: \hyperlink{https://am.globalvoices.org}{Amharic}, \hyperlink{https://ig.globalvoices.org}{Igbo}, \hyperlink{https://mg.globalvoices.org}{Malagasy}, \hyperlink{https://sw.globalvoices.org}{Swahili}, and \hyperlink{https://yo.globalvoices.org}{Yoruba}.
% \subsubsection{DW}
% We collected data for \hyperlink{https://www.dw.com/am/ይዘት/s-11646}{
% Amharic}, \hyperlink{https://www.dw.com/ha/batutuwa/s-11603}{Hausa} and \hyperlink{https://www.dw.com/sw/idhaa-ya-kiswahili/s-11588}{Swahili}.
% \subsubsection{Online Newspapers}
% We collected multiple online newspapers in $14$ African languages. We provide a table detailing the various newspapers we crawled for each language in Table XX.
\subsection{Existing Corpora}
We collected corpora available on the web for different African languages. We collected data \hyperlink{https://www.gutenberg.org/browse/languages/af}{Project Gutenberg} for Afrikaans, \hyperlink{https://zenodo.org/record/3668495#.YcTXu2DMJyy}{South African News data} for Sepedi and Setswana, OSCAR \cite{AbadjiOrtizSuarezRomaryetal.2021} for Afrikaans, Amharic, Somali, Swahili, Oromo, Malagasy, and Yoruba. We also used \hyperlink{https://opus.nlpl.eu/Tatoeba.php}{Tatoeba} for Afrikaans, Amharic, Bemba, Igbo, Kanuri, Kongo, Luganda, malagasy, Sepedi, Ndebele, Kinyarwanda, Somali, Swahili, Tsonga, Xhosa, Yoruba and Zulu; \hyperlink{https://zenodo.org/record/3553423#.YcTXkWDMJyx}{Swahili Language Modelling Data} for Swahili; \hyperlink{https://github.com/ijdutse/hausa-corpus/blob/master/data/all-merged-hausa-datasets.txt}{Ijdutse corpus} for  Hausa; \hyperlink{https://github.com/AI-Lab-Makerere/Data4Good}{Data4Good corpora} for Luganda, CC-100 for Amharic, Fulah, Igbo, Yoruba, Hausa, Tswana, Lingala, Luganada, Afrikaans, Somali, Swahili, Swati, North Sotho, Oromo, Wolof, Xhosa, and Zulu; \hyperlink{https://huggingface.co/datasets/castorini/afriberta-corpus}{Afriberta-Corpus} for Afaan / Oromo, Amharic, Gahuza, Hausa, Igbo, Pidgin, Somali, Swahili, Tigrinya and Yoruba; \hyperlink{https://huggingface.co/datasets/mc4}{mC4} for Afrikaans, Amharic, Hausa, Igbo, Malagasy, Chichewa, Shona, Somali, Sepedi, Swahili, Xhosa, Yoruba and Zulu. 
\subsection{Government Documents}
Government documents were retrieved from \hyperlink{https://www.sadilar.org/index.php/en/}{South African Centre for Digital Language Resources} (SADiLaR), and the \hyperlink{https://www.ohchr.org/en/udhr/pages/searchbylang.aspx}{Universal Declaration of human rights} (UDHR) documents in multiple languages.

% \subsubsection{SADiLaR}
% SADiLaR provides infrastructure including models and data for South African indigenous languages. Although, a few resources are available for English and other African languages. We collected all text data available on SADiLaR for the 10 African languages including: Afrikaans, IsiNdebele, IsiXhosa, IsiZulu, Sepedi, Sesotho, Setswana, Siswati, Tshivenda, and Xitsonga. 
% \subsubsection{UDHR}
% The UDHR document is available in 530 different translations. We collected translations for 102 African languages / dialects. 
% \subsection{Internet Crawls}

\subsection{Health Documents}
We collected multiple health documents from the Department of Health, State Government of Victoria, Australia. We collected documents in Amharic, Dinka, Harari, Oromo, Somali, Swahili, and Tigrinya. 

\subsection{Preprocessing}
Preprocessing involved using langid.py to discriminate high resource languages in our datasets. We were interested in identifying English, French, Portuguese, and Arabic - which are the most commonly used foreign languages in Africa. This was to ensure that our data contained only indigenous African languages. Next we tokenized using whitespace only. This because there are no high quality language specific tokenizers available for the languages we train. We learned BPE using subwordNMT \cite{sennrich-etal-2016-neural} and used 100K merge operations. The BPE codes are learned on the concatenation of sentences sampled from all languages. We also created character based tokens to train our character level models.

\subsection{Evaluation data for Pretraining}
We evaluated our model using data that we did not include in the training. We used the following datasets: 

%\begin{table}[h!]
%\small 
%\centering
%\begin{tabular}{>r{2}r{2}r{2}} 
%\begin{tabular}{>{}c|l r}
% \toprule
%\multicolumn{1}{c}{}  &\textbf{Organization} & \textbf{Type} \\ 
% \midrule
%\multicolumn{1}{c}{}  &\href{https://www.google.org/}{Google} & Industry  \\
%\multicolumn{1}{c}{}  &\href{https://www.microsoft.com/en-ca/about/}{Microsoft} & Industry  \\
%\multicolumn{1}{c}{}  &\href{https://www.rockefellerfoundation.org/commitment/innovation/}{The Rockefeller Foundation} & Foundation   \\
%\multicolumn{1}{c}{}  &\href{https://www.rockefellerfoundation.org/commitment/innovation/}{FAIR Forward} & Government  \\
%\multicolumn{1}{c}{}  & \href{https://lacunafund.org/}{Lacuna Funds} & NGO\\
%\multicolumn{1}{c}{}  & \href{https://www.k4all.org/}{Knowledge 4 All} & Research \\
%\multicolumn{1}{c}{}  & \href{https://www.idrc.ca/en}{IDRC} & Research  \\
% \bottomrule
%\end{tabular}
%\caption{Some funding Organization for African NLP including Non-Governmental organizations (NGO)s}\label{tab:funding}
%\end{table}

==> to-do.tex <==
Evaluation 
code-switching - code-switched African languages translated to any language. prompting generation - prompting commands
Bias /fairness generation - analyze data to determine the bias
Benchmark - release all benchmark data (like superglue)

